Harnessing the Power of Infinitely Wide Deep Nets on Small-data Tasks

Recent research shows that the following two models are equivalent: (a) infinitely wide neural networks (NNs) trained under l2 loss by gradient descent with infinitesimally small learning rate (b) kernel regression with respect to so-called Neural Tangent Kernels (NTKs) (Jacot et al., 2018). An efficient algorithm to compute the NTK, as well as its convolutional counterparts, appears in Arora et al. (2019a), which allowed studying performance of infinitely wide nets on datasets like CIFAR-10. However, super-quadratic running time of kernel methods makes them best suited for small-data tasks. We report results suggesting neural tangent kernels perform strongly on low-data tasks. 1. On a standard testbed of classification/regression tasks from the UCI database, NTK SVM beats the previous gold standard, Random Forests (RF), and also the corresponding finite nets. 2. On CIFAR-10 with 10 - 640 training samples, Convolutional NTK consistently beats ResNet-34 by 1% - 3%. 3. On VOC07 testbed for few-shot image classification tasks on ImageNet with transfer learning (Goyal et al., 2019), replacing the linear SVM currently used with a Convolutional NTK SVM consistently improves performance. 4. Comparing the performance of NTK with the finite-width net it was derived from, NTK behavior starts at lower net widths than suggested by theoretical analysis(Arora et al., 2019a). NTK's efficacy may trace to lower variance of output.

==> oldintro.tex <==
%Over-parameterized neural networks, optimization and generalization mystery
A key feature in recent success of deep learning is that modern neural networks (NNs) are highly over-parameterized, i.e., the number of parameters is much larger than the number of training samples.
These over-parameterized NNs not only can fit all training data, a.k.a., achieving zero training error but also, contrary to the classical learning theory point of view, enjoy low generalization error in practice~\citep{zhang2016understanding}.


%Over-parameterized neural networks and NTKs
A recent line of theoretical results on over-parameterized neural networks suggest the equivalence between a fully-trained neural network predictor and a kernel predictor with particular kernel, neural tangent kernel (NTK)~\citep{jacot2018neural}.
Theoretically, researchers used this connection to prove the global convergence of gradient to achieve zero training error~\citep{du2018gradient,du2018deep} and explained the generalization behavior of over-parameterized neural networks as one can just use existing generalization bounds of kernel predictors~\citep{arora2019fine,arora2019exact}.
See Section~\ref{sec:rel} for a more discussions.



%advantages of NTK comparing to NN
From a practical point of view, this connection suggests a promising new class of predictors.
Since every neural network architecture corresponds to a kernel function, one can just try out this kernel predictor.
Kernel predictors have several advantages comparing to NN predictors.
For optimization, kernel predictor is much easier to train as one just needs to solve a convex program and there are existing stable solvers whereas NNs often require tuning hyper-parameters of the gradient-based optimization algorithms.
Furthermore, training NN requires random initialization and stochastic training algorithms and thus NN has more variance than the kernel predictor.


%there is still a gap between neural networks and NTKs
Nevertheless, NTKs often perform worse than their corresponding NNs on \emph{large scale} data.
\citet{arora2019exact} conducted experiments comparing convolutional neural networks (CNNs) and their kernel counter parts, convolutional neural tangent kernels (CNTKs) and observed CNNs often enjoy $5-6\%$ better test accuracy than their corresponding CNTKs.\footnote{CNNs used in \cite{arora2019exact} turned off batch norm, weight decay, so the only the finite width and/or optimization procedure can account for the performance difference. }
%A key feature of these requires the width to be a large polynomial in $n$ where in practice.
%For large scale benchmark datasets, like CIFAR and Imagenet, the width of the convolutional neural network it is often smaller than $n$.
From theoretical point view, the performance gap is not unexpected.
All existing theoretical work that establish the equivalence between NNs and NTKs require the width $m$ (number of neurons for fully-connect NNs or number of channels for CNNs) at least a large polynomial in the number of data $n$.
For example, the current best bound for the shallow two-layer neural network requires $m = O(n^4)$~\citep{song2019quadratic}. \footnote{We remark that the width is small does not contradict with the fact that the neural networks are highly over-parameterized as these over-parameterized NNs often have multiple layers.}

%On small data sets
What about small data sets?
A recent work empirically study the performance of neural networks on small datasets~\citep{olson2018modern}.
They used a fixed architecture and show modern deep neural networks are competitive with random forest (RF), though there is still a performance gap from RF predictor.
Since the theory suggests if $n$ is small, then NTK is a good approximation to the learned NN, we expect NTK predictor may perform better or at least on par with NN predictors.
Another small data regime where NTK  can be helpful is the low-shot learning where the standard strategy is to use a pre-treained neural network to extract feature then apply a linear classifier~\citep{goyal2019scaling}.
For this setting, NTK can be used as drop-in component to replace the linear classifier.

The current paper studies the following question:
\begin{center}
%	\textbf{Q1: In the small data regime, how well do NTKs approximate NNs?}\\
	\textbf{In the small data regime, how well do NTKs perform?}
\end{center}
We perform extensive experiments on $90$ classification tasks from UCI database, an image classification on a sub-sampled CIFAR 10 dataset and a low-shot image classification task on VOC07 with transfer learning to give a strong positive answer to the above question.
\simon{@Sanjeev: for UCI data we only select number of training data $<5000$ and ignore all datasets that have explicit training / testing split because we found there is often a big difference between training and testing.}
Our main findings are summarized below:
\begin{itemize*}
	\item NTK predictor achieves superior, and arguably the strongest classification performance. This is verified via several standard statistical tests, including Friedman rank, average accuracy, 
%	Cohen's $\kappa$, 
	Percentage of maximum accuracy (PMA) and probability of achieving 90\%/95\% maximum accuracy (P90 and P95), performed to compare performances of different classifiers on $90$ datasets from UCI database.
	Our experiment suggests NTK can be the new ``gold standard" on small datasets and can be directly use as an off-the-shelf classifier.

%	\item Via pairwise comparisons, we find NTK often performs better than other strong classifiers, e.g.,  random forest and kernel SVM, on datasets with low Bayes error.
	
	\item NTK is indeed a good approximation for NN in the small data regime. 
	As on $90$ UCI datasets, we find for all datasets, the difference between NN and NTK is within $5\%$ whereas there exists that the difference between other classifier like RF and NTK (or NN) is large ($>20\%$).
	Comparing NTK and NN, NTK is more stable (smaller variance), which explains why in general NTK enjoys better accuracy than NN on small datasets (cf. Figure~\ref{fig:nn_ntk})
%	 and 2) when $L_2$ loss is used, the final predictions of NTK and NN are quite close.
%	We also observe as the width becomes larger, NN prediction is closer to NTK, thus verifying the recent theoretical development.
	\item \simon{to incorporate after the experiments are done}Small CIFAR 10.
	\item NTK can be used as a drop-in method in low-shot learning. We show on the low-shot image classification task on VOC07 with feature extracted from ResNet50 trained on ImageNet, replacing the linear classifier with CNTK consitently improve the performance.
	Therefore, we believe NTK (or CNTK for image data) can be used as standard component for low-shot learning.
\end{itemize*}





\paragraph{Organization}
This paper is organized as follows.
In Section~\ref{sec:rel}, we discuss related work.
In Section~\ref{sec:pre}, we review the derivation of NTK.
In Section~\ref{sec:exp_uci}, we present our experimental findings about NN and NTK on UCI dataset.
In Section~\ref{sec:exp_cifar}, we present our experiment findings about CNN and CNTK on small CIFAR dataset.
In Section~\ref{sec:exp_transfer}, we present our experiment findings about CNTK for the low-shot learning setting.
We conclude in Section and put some additional technical details in appendix.







